dpBento: Benchmarking DPUs for Data Processing

Data processing units (DPUs, SoC-based SmartNICs) are emerging data center hardware that provide opportunities to address cloud data processing challenges. Their onboard compute, memory, network, and auxiliary storage can be leveraged to offload a variety of data processing tasks. Although recent work shows promising benefits of DPU offloading for specific operations, a comprehensive view of the implications of DPUs for data processing is missing. Benchmarking can help, but existing benchmark tools lack the focus on data processing and are limited to specific DPUs. In this paper, we present dpBento, a benchmark suite that aims to uncover the performance characteristics of different DPU resources and different DPUs, and the performance implications of offloading a wide range of data processing operations and systems to DPUs. It provides an abstraction for automated performance testing and reporting and is easily extensible. We use dpBento to measure recent DPUs, present our benchmarking results, and highlight insights into the potential benefits of DPU offloading for data processing.

==> Evaluations/ML.tex <==
% \subsection{Machine Learning \TODO{JH}}
% \label{sec:ML}

% Machine Learning workloads including image classifications.

\if 0
\begin{table} [h]
\small
\setlength{\tabcolsep}{5pt}
    % \caption{Parameters for network benchmarking.}
    \centering
    \begin{tabular}{c c}
        \toprule
        {\bf Scale Factor} & {\bf Query}  & {\bf \#Threads} \\
         \midrule
        10 &
        Q1--Q9 &
        Max\\
        \bottomrule
    \end{tabular}
    \label{tab:graph-setup}
\end{table}
\fi

% We examine the DPUs' capabilities in machine learning under the context of lightweight inference workloads. Figure \ref{fig:ml-img-classification-fp32} demonstrates the performances of the DPU SoCs and the host CPU, where we focus on the inference throughput of image classification. In a single thread scenario, the host CPU offers far better latency, but as the number of threads used starts increasing, the percentage performance gains are in favor of the DPUs, although the host CPU still holds a sizable advantage.
% The \nvbff performance is especially competitive compared to \nvbf and \octeon, which constantly achieves more than double the throughput with different parallelism. The host CPU cannot fully exploit its core count and scales poorly with a larger number of threads, likely due to the small size and architecture of the model involved; by contrast, the \octeon DPU scales positively to its full 24 cores, we deduce that this is because of the relatively low throughput and weaker per core computing power.
% Using a quantized version of the same model (\verb|int8| vs. \verb|fp32|), we observe throughput gains across all platforms as expected of quantization; the performance gap between \nvbff and the host also remains at a similar level---\nvbff's peak throughput is approximately 55\% of the host's, however, \nvbff needs only 8 threads to achieve peak throughput with \verb|int8| compared to 16 with \verb|fp32|. And similarly, the host cannot benefit from its much higher core count, achieving peaking throughput with 8 threads as well.
% The BlueField-3 is much more competitive compared to the other DPUs, and offers arguably the same level (single-digit ms) of performance the host CPU can offer.


\if 0
\begin{figure}[t]
    \begin{minipage}{1\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ml/ml-480p-fp32-diff_threads.pdf}
        \caption{\TOCHECK{Image classification throughput, EfficientNet-B0, fp32 model w/ LiteRT framework}}
        \label{fig:ml-img-classification-fp32}
    \end{minipage}
\end{figure}

\begin{figure}[t]
    \begin{minipage}{1\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ml/ml-480p-int8-diff_threads.pdf}
        \caption{\TOCHECK{Image classification throughput, EfficientNet-B0, quantized int8 model w/ LiteRT framework}}
        \label{fig:ml-img-classification-int8}
    \end{minipage}
\end{figure}
\fi

% \begin{figure}[t]
%     \begin{minipage}{1\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/ml/ml-1080p-int8-vs-fp32.pdf}
%         \caption{Quantization effect on different platform processors, for image classification task using EfficientNet with LiteRT}
%         \label{fig:ml-img-classification-quantization}
%     \end{minipage}
% \end{figure}

==> Evaluations/graph.tex <==
\subsection{Graph Processing and ML}
\label{sec:graph-processing}

\begin{table} [t]
\small
\setlength{\tabcolsep}{5pt}
    \caption{Parameters for graph processing and ML.}
    \centering
    \begin{tabular}{c c c c c}
        \toprule
        \multicolumn{3}{c}{\bf Graph Processing} &  \multicolumn{2}{c}{\bf Machine Learning} \\\midrule
        {\bf Graph size} & {\bf Query}  & {\bf \#Threads} & {\bf Precision} & {\bf \#Threads}\\
        \midrule
        1\,GB &
        Q1--Q9 &
        Max &
        {\tt int8}, {\tt fp32} &
        Max\\
        \bottomrule
    \end{tabular}
    \label{tab:graph-setup}
\end{table}

\begin{figure}[b]
\centering
\begin{minipage}[t]{0.64\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{images/graph/graph.pdf}
    \caption{Graph processing.}
    \label{fig:graph}
\end{minipage}
\hfill
\begin{minipage}[t]{0.32\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{images/ml/ml.pdf}
    \caption{ML.}
    \label{fig:ml}
\end{minipage}
\end{figure}

The parameters for benchmarking lightweight graph processing and ML performance with Kuzu and LiteRT are in Table~\ref{tab:graph-setup}.
For Kuzu, we let the system consume all the cores and measure its running times of all queries in the LSQB benchmark.
Figure~\ref{fig:graph} shows the benchmark results.
On average, the DPU takes 2.9$\times$ longer time to complete the graph queries.
The slowdown of the DPU relative to the host greatly varies between queries.
For instance, the DPU achieves the same performance as the host for Q4, but is 8$\times $ slower for Q6.
Q3 and Q9 are much slower than other queries on both platforms.
For instance, Q3 computes triangles in the input graph and takes several hours to complete on the DPU.

In the ML experiments, we measure the inference speed (images/s) on the DPU and the host (utilizing all available cores) with different model parameter precisions.
Figure~\ref{fig:ml} demonstrates performance of the DPU and the host.
When the model is quantized with {\tt int8}, LiteRT processes 217 images/s on the host vs. 123 images/s on the DPU---a 44\% throughput degradation on the DPU.
When adopting the model with {\tt fp32}, while the throughput of both platforms drops, benefiting from higher efficiency in processing floating-points (Section~\ref{sec:comp-primitive}), the degradation is milder on the DPU: 16\%, compared to 23\% on the host.

\vspace{3mm}
\begin{mdframed}[style=FindingFrame,nobreak=false,align=center,userdefinedwidth=27em]

{\em Compared to other data processing tasks, graph queries present diverse performance characteristics on the DPU: some queries complete as quickly as on the host, but some are hopelessly slower.}

{\em For ML inference, the performance degradation on the DPU is lower with floating-point models.
On average, the DPU performance gap to host  is consistently noticeable in all benchmarked systems.}

\end{mdframed}


% In general, we see that BF-3 is 2-4x faster than BF-2 and that FN1 is 2-3x faster than BF-3, which falls roughly in line with their CPU performance (BF-3 having twice as many cores as BF-2 and the cores being 5 generations newer, and FN1 having 1.5x as many cores as BF-2, being multithreaded, and being a server CPU). For query 3, (finding triangles in the graph) we suspect that Kuzu isn't parallelzing the query right now (but this can change in the future), leading to a long runtime. Query 9 is similar in needing to traverse the entire graph. Q4 being slower on FN1 compared to BF-3 is probably a dis-economy of scale. Reducing the number of threads to 24 on FN1 reduced the cold runtime to 0.
% 983 seconds and the hot runtime was 0.678 seconds. 

==> Evaluations/kv-store.tex <==
\subsection{Key-Value Store}
\label{sec:kv-store}

To test KV operations on the DPUs, we use the following parameters to vary operation type and access distribution on a 10\,GB database of 1\,KB KV records.
As in the previous systems, we let RocksDB utilize all available cores on the platform.

\begin{table} [h]
\small
\setlength{\tabcolsep}{1pt}
    % \caption{Parameters for network benchmarking.}
    \centering
    \begin{tabular}{c c c c c}
        \toprule
        {\bf Scale} & {\bf Record Size} & {\bf Operation}  & {\bf Distribution}  & {\bf \#Threads} \\
        \midrule
        10\,GB &
        1\,KB &
        100\% R, 50\% R+50\% W &
        Uniform, Skewed &
        Max\\
        \bottomrule
    \end{tabular}
    \label{tab:kvs-setup}
\end{table}


\begin{figure}[t]
    \centering
    \begin{subfigure}{.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{images/kvs/kv-thr.pdf}
        \caption{Throughput.}
        \label{fig:kv-thr}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{.49\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{images/kvs/kv-lat.pdf}
        \caption{Latency (average and p99).}
        \label{fig:kv-lat}
    \end{subfigure}
    \caption{Benchmarking KV performance.}
    \label{fig:kv}
\end{figure}

Due to space limit, from this section, we focus on comparing the host and \nvbff to show the state-of-the-art DPU performance.
Figure~\ref{fig:kv-lat} reports the throughput achieved by the DPU and the host on different workloads (pure reads vs. mixed reads and writes) and access patterns (uniform vs. zipfian $\theta=0.99$).
As it behaves on the host, the throughput of skewed accesses in RocksDB is slightly higher than that of uniform accesses, and the throughput of pure reads is significantly higher than the mixed workload.
However, compared to the host, RocksDB experiences 50\%--60\% throughput drop on the DPU.
We also observe that the throughput drop from the read workload to the mixed workload is more substantial on the DPU because the  performance gap of writes between the DPU and the host is larger than that of reads, as presented in Section~\ref{sec:stor}.
Figure~\ref{fig:kv-lat} shows the average and tail latency of RocksDB, which is generally 2$\times$ higher on the DPU than the host latency.

\vspace{3mm}
\begin{mdframed}[style=FindingFrame,nobreak=false,align=center,userdefinedwidth=27em]

{\em In summary, RocksDB consistently experiences significant performance degradation on the DPU compared to the host, for both throughput and latency.
In addition, reads are better candidates for DPU offloading than writes.}

\end{mdframed}


==> Makefile <==
###########################################################
#0;136;0c
# Makefile for LaTeX docs
#
# $Id:
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

#all: eps dvi ps pdf # res
all: pdf
eps: fig obj

#PAPER=mosaic
PAPER=paper
#PAPER=vldb_sample

LATEX=pdflatex

ps:  $(PAPER).ps

pdf: $(PAPER).pdf
dvi: $(PAPER).dvi

obj: $(patsubst %.obj, %.eps, $(wildcard *.obj))
fig: $(patsubst %.fig, %.eps, $(wildcard *.fig))

res:
	make -C results
	make -C figs

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

# only need -Ppdf if using CM fonts
#%.pdf: %.dvi $(wildcard *.bib)
#	dvips -Ppdf -G0 -t letter -o $*.tmp.ps $<
#	ps2pdf $*.tmp.ps $*.pdf
#	$(RM) $*.tmp.ps $*.dvi *.aux *.log *.bbl *.blg *.toc

%.pdf: $(wildcard *.tex) $(wildcard *.bib)
	$(LATEX) $*
	bibtex $*
	$(LATEX) $*
	if [ -e $*.toc ] ; then $(LATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	#dvips -t letter -z -Ppdf -G0 -D600 main.dvi -o main.ps
	#ps2pdf main.ps main.pdf

	$(RM) *.aux *.log *.blg *.toc

%.ps: %.dvi
	dvips -Ppdf -G0 -tletter -o $@ $<
%.ps.gz: %.ps
	gzip -v9 $<

%.eps: %.obj
	tgif -print -eps $*

%.eps: %.fig
	fig2dev -L eps $< $@


==> bf3.tex <==
\section{NVIDIA BlueField}
\label{sec:nvidia-bf}
\todo{paper writing} partition by workload, not by different DPUs here
Present benchmarking results on BlueField-2 \& BlueField-3

% \subsection{Hardware Specification}
% \todo{JH}

% Introduce BF-2\&3 here

\subsection{Result Analysis}

\subsubsection{Compute}
\todo{JH}

\subsubsection{Memory}
\todo{RV}

\subsubsection{Storage}
\todo{CC}

\subsubsection{Networking}
\todo{AL}

\subsubsection{DBMS}
\todo{YC}

\subsubsection{KV Store}
\todo{YC}

\subsubsection{Graph databases}
\todo{YC \& RV}

% \subsubsection{MapReduce}
% \todo{CC \& AL}

\subsubsection{ML}
\todo{JH}



==> composition.tex <==
\section{Composition}
\label{sec:comp}

Present results with a composed SPJA (scan-project-join-aggregation) query and see how the previous findings can be applied.
Specifically, we generate the query plans from the 22 TPC-H queries and find sub-queries that follow the SPJA pattern, and then evaluate them accordingly.

==> discuss.tex <==
\section{Discussions \TODO{All}}
\label{sec:discuss}

Compare BF-3 and IPU performance and our future directions

==> pensando.tex <==
\section{AMD Pensando}
\label{sec:pensando}

Present benchmarking results on recent AMD Pensando

% \subsection{Hardware Specification}
% \todo{JH}

Introduce Pensando here

\subsection{Result Analysis}

\subsubsection{Compute}
\todo{JH}

\subsubsection{Memory}
\todo{RV}

\subsubsection{Storage}
\todo{CC}

\subsubsection{Networking}
\todo{AL}

\subsubsection{DBMS}
\todo{YC}

\subsubsection{KV Store}
\todo{YC}

\subsubsection{Graph databases}
\todo{YC \& RV}

% \subsubsection{MapReduce}
% \todo{CC \& AL}

\subsubsection{ML}
\todo{JH}


